Weakly Supervised Human-Object Interaction Detection in Video via Contrastive Spatiotemporal Regions

We introduce the task of weakly supervised learning for detecting human and object interactions in videos. Our task poses unique challenges as a system does not know what types of human-object interactions are present in a video or the actual spatiotemporal location of the human and the object. To address these challenges, we introduce a contrastive weakly supervised training loss that aims to jointly associate spatiotemporal regions in a video with an action and object vocabulary and encourage temporal continuity of the visual appearance of moving objects as a form of self-supervision. To train our model, we introduce a dataset comprising over 6.5k videos with human-object interaction annotations that have been semi-automatically curated from sentence captions associated with the videos. We demonstrate improved performance over weakly supervised baselines adapted to our task on our video dataset.

==> fig_text/attention_model.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.5\textwidth]{fig/attention_model3.pdf}
\end{center}
\caption{ \small{Attention model.}}
\label{fig:attention_model}
\end{figure}


==> fig_text/pipeline.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{fig/model_overview.pdf}
\end{center}
\caption{\small \textbf{An overview of the proposed method during training.} We take video frames as input and send them to a temporal soft attention module and a feature aggregation module. The output features incorporate the temporal and spatial information and are combined with the feature of a human-object interaction label to compute the spatiotemporal loss.
}
\label{fig:model_architecture}
\end{figure}





% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=1\linewidth]{fig/model_pipeline6.pdf}
% \end{center}
% \vspace{-18pt}
% \caption{\small Model architecture of the proposed method. (a) is the overview of the training process. We take video frames as input and send them to a temporal soft attention module and a feature aggregation module. The output features incorporate the temporal and spatial information and are used to compute the spatiotemporal loss. 
% (b) is the illustration of the feature aggregation module.
% In each frame, we use the Faster-RCNN/Densepose to extract the object and human region proposal locations and an ROI pooling layer to extract their features. The object/human score functions take the feature of a region proposal from the ROI pooling layer, the language phrase, and the frame feature $x'_t$ (do not show here) as input and output a score for the region. We aggregate the object/human region proposal features based on their scores from the score function to generate the aggregated object/human features.
% }
% \label{fig:model_architecture}
% \vspace{-20pt}
% \end{figure}



% Model architecture of the proposed method. (a) is the overview of the training process. We take video frames as input and send them to a temporal soft attention module and a feature aggregation module. The output features incorporate the temporal and spatial information and are used to compute the spatiotemporal loss. (b) is an illustration of the feature aggregation module. For each frame, it takes the frame feature $x'_t$, the language query, and the RGB frame as input and output the aggregated features of human and object region proposals used in (a). (c) shows the temporal soft attention module in (a) and the score function in (b). In the soft attention module, we use the temporal information to learn frame features. The score function concatenates the features from $x'_t$, the language input, and the feature of each human/object region proposal and generate a score for each region proposal. See text for more details.

% Model architecture of the proposed method. (a) is the overview of the training process. We take video frames as input and send them to a temporal soft attention module and a feature aggregation module. The output features incorporate the temporal and spatial information and are used to compute the spatiotemporal loss. (b) is an illustration of the feature aggregation module. For each frame, it takes the frame feature $x'_t$, the language query, and the RGB frame as input. The RGB frame is sent to Densepose/Faster-RCNN followed by an ROL pooling layer to extract human/object proposal features. The score function generates a score for each human/object region proposal to evaluate their probability of being the query action/object. A feature aggregation layer aggregates the features of human/object region proposals to compute the spatiotemporal loss in (a). (c) shows the temporal soft attention module in (a) and the score function in (b). In the soft attention module, we use the temporal information to learn frame features. The score function concatenates the features from $x'_t$, the language input, and the feature of each human/object region proposal and generate a score for each region proposal.


% Model architecture of the proposed method. (a) is the overview of how to train our model. We take a series of video frames as input and send them to a temporal soft attention module and a feature aggregation module to incorporate the temporal and spatial information when computing the spatiotemporal loss. (b) is an illustration of the feature aggregation module. For each frame, it takes the frame feature $x'_t$, language query and original frame as input. The image is first sent to Densepose/Faster-RCNN to extract the human/object region proposals and then an ROL pooling layer is applied to the region proposals to extract their features. Each human/object region proposal has a score to evaluate their probability of being the query action/object through a score function. A feature aggregation layer aggregate the features of human/object region proposals to compute the spatiotemporal loss in (a). (c) shows the temporal soft attention module in (a) and the score function in (b). In the soft attention module, a frame $x_t$ is sent to an embedding layer to generate a query vector and combined with the key and value vectors generated by other frames in the same video to obtain a new frame feature $x'_t$ that contains the temporal information. The score function concatenates the features from $x'_t$, the language input, and the feature of each human/object region proposal and generate a score for each proposal through an MLP layer.

==> fig_text/soft_attention.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{fig/soft_attention4.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Illustration of the temporal soft attention and score function. In the soft attention module, we use the temporal information to learn frame features. The score function takes the frame feature $x'_t$, the language input, and each human/object region proposal feature to generate a score for each region proposal.}
\label{fig:soft_attention}
\vspace{-10pt}
\end{figure}




==> fig_text/testing_overview.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.5\textwidth]{fig/testing_overview.pdf}
\end{center}
\caption{ \small{Inference model.}}
\label{fig:testing_overview}
\end{figure}


==> fig_text/video_loss.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.75\linewidth]{fig/video_loss.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Illustration of the temporal consistency module. Given several frames of video, we compute the bounding box with the highest attention weight in each image. We use N-pairs contrastive loss to encourage the representation of each box to be similar to the highest weight box in other frame and to be different from other bounding boxes in the same frame. This essentially encourages the most confident detection to be consistent through time.}
\label{fig:video_loss}
\vspace{-10pt}
\end{figure*}




==> table/hicodet.tex <==

\begin{table}[t]
\scriptsize
\caption{\small Evaluation of performance on HICO-DET compared to methods in \cite{peyre2017weakly}, \cite{zhou2018weakly} and different random baselines. Phrase detection refers to correct localization (0.5 IoU) of the union of human and object bounding boxes while relationship refers to correct localization of both human and object bounding boxes. 
% See \sect{sect:metrics} for introduction of metrics.
}
\label{tbl:hicodat}
\begin{center}
\setlength{\tabcolsep}{2pt}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|cccc|cc}
\toprule
\bf Model & \multicolumn{4}{c|}{\bf mAP (\%)} & \multicolumn{2}{c}{\bf Recall@1 (\%)} \\
\midrule
& Phr (ko) & Rel (ko) & Phr (def) &  Rel (def) & Phr & Rel \\
\midrule
Ours Random  & 9.12 & 0.71 &&& +13.61 & +0.32 \\
Ours Random Pretrain & 10.31 & 0.75	&&& +14.70 & +0.90		\\
Peyre2017 \cite{peyre2017weakly} & 27.11 & 3.25 &&& 34.54 & 1.50  \\
Zhou2018 \cite{zhou2018weakly}  & 11.94 &  2.70 &&& 42.88 & 8.50 \\
\midrule
Ours & \bf 58.37 & \bf 13.10	&&& +42.25 & +7.01		\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}



==> text/introduction_new.tex <==
\vspace{-2pt}
\section{Introduction}
\vspace{-2pt}
To understand the visual world around us, a machine must not only be able to segment the individual objects in a scene, but also the interactions between them. Humans often form the core of such interactions, and so in this paper, we study the problem of Human-Object Interaction (HOI) in videos. 
Given a video sequence, as illustrated in Figure~\ref{fig:teaser_video}, a system must correctly identify and localize the person and interacted object (``horse’’) in the scene, in addition to identifying the action (``grooming’’) taken by the human, for the duration of the interaction in the video. 
Achieving such a goal has many important applications, such as video retrieval, surveillance or human-robot interaction. 

\input{fig_text/teaser.tex}

Previous human-object interaction detection methods \cite{chao2018learning,chao2015hico,gupta2015visual,hou2020visual,wang2020discovering,wang2019deep,qi2018learning,xu2019learning,zhou2019relation,wan2019pose,song2020novel} 
% have focused mainly on still images. 
are based on the context of still images. 
However, human-object interactions are temporal events and occur over a period of time. 
Interactions such as ``drinking’’ or ``pushing’’ 
are temporal interactions between a human and an object, making videos a natural modality where to study this problem. 
% symbolize temporal interaction between human and object, making videos a more natural way to study this problem.
Most existing video-based methods are based on supervised learning which relies on large-scale fully annotated video datasets. However, such approaches suffer several significant drawbacks in the human-object interaction detection problem. 
% Most existing human-object interaction approaches \cite{chao2018learning,gao2018ican,gupta2015visual} are further typically fully supervised, which suffers from several significant drawbacks. 
First, exhaustively annotating objects in video is time consuming given the large number of frames in a video. 
Second, scaling to the large number of possible interactions and obtaining a sufficient amount of ground truth bounding boxes for supervised learning is challenging due to the potentially open vocabulary of objects and actions and the combinatorial nature of human-object interactions. 
Third, interactions typically follow a long-tailed distribution, with common human-object interactions, such as human riding horse, occurring much more prevalently than others, such as human riding zebra \cite{yuhang2020novel,hou2020visual}. While supervised learning usually prefers common interactions, a robust human-object interaction detection system should instead perform equally well on both common and rare interactions. 


In this work, we seek to leverage videos with just verb and noun phrase annotations derived from natural language sentence captions to learn how to detect HOIs in videos. Such an approach is advantageous as obtaining video-level annotations is significantly less costly than bounding boxes in each frame. 
Leveraging such data makes it possible to scale training to larger number of videos and toward an open vocabulary of objects and actions. 


As bounding box annotations are not available in captioned videos, our goal is to detect a human and an object interacting in a video in a weakly supervised fashion without the usage of bounding box annotations. This goal is challenging as we do not know what type of human-object interaction is present in a given video and what are the spatiotemporal locations of humans and objects that depict the undergoing interactions.
Moreover, in contrast to previous work detecting interactions with fixed vocabulary~\cite{Shang2017VideoVR,tsai2019GSTEG}, our method is able to leverage the pretrained language model to detect unseen human-object interactions in the open vocabulary during testing.
% the set of ``in-the-wild’’ actions and objects may span a large, open vocabulary.


As one of our technical contributions, we introduce a weakly supervised spatiotemporal training loss for our task. 
Our loss aims to jointly associate candidate spatiotemporal regions with an action and object vocabulary and leverages cues about the temporal continuity of objects in motion. 
Given weak supervision in the form of an action and object during training, our loss encourages the visual representation for likely human and object spatiotemporal regions to be close to the corresponding language embedding representation of the input action and object query. 
Such a formulation allows our approach to deal with an open vocabulary of language queries. This is especially desirable in human-object interaction detection, due to the high prevalence of rare and unseen action and object combinations. We show that such an approach enables us to detect interactions consisting of new unknown objects.
The loss also maintains temporal continuity of the object's visual appearance throughout the video. 
% Moreover, our loss contrasts the spatiotemporal region's visual appearance against language-embedding representations of other words in the action or object vocabulary and against other spatiotemporal regions in the video. 


% To enable human-object interaction detection in videos, we introduce a dataset of over 6k videos derived from the Moments in Time dataset~\cite{monfort2019moments} where human-object interactions have been semi-automatically curated from natural language captions accompanying the videos. 


Our paper has three main contributions: 
(1) We present an approach that integrates the spatial, temporal, human, and object information for weakly supervised human-object interaction detection in videos and avoids the time-consuming video annotation.
(2) We present a spatiotemporal loss that enables us to handle the human-object interactions with long-tailed distribution, and further allows us to detect interactions involving new unknown objects in a zero-shot manner.
(3) We introduce a new dataset of over 6k videos to evaluate human-object interaction in videos. We demonstrate improved performance over weakly supervised baselines adapted to our task.

